Navigating the Post-API Dilemma | Search Engine Results Pages Present a Biased View of Social Media Data

Recent decisions to discontinue access to social media APIs are having detrimental effects on Internet research and the field of computational social science as a whole. This lack of access to data has been dubbed the Post-API era of Internet research. Fortunately, popular search engines have the means to crawl, capture, and surface social media data on their Search Engine Results Pages (SERP) if provided the proper search query, and may provide a solution to this dilemma. In the present work we ask: does SERP provide a complete and unbiased sample of social media data? Is SERP a viable alternative to direct API-access? To answer these questions, we perform a comparative analysis between (Google) SERP results and nonsampled data from Reddit and Twitter/X. We find that SERP results are highly biased in favor of popular posts; against political, pornographic, and vulgar posts; are more positive in their sentiment; and have large topical gaps. Overall, we conclude that SERP is not a viable alternative to social media API access.

==> images/reddit_rtd.tex <==



\begin{tikzpicture}
	\begin{axis}[
        width=\linewidth,
        height=2.5in,
        title={Reddit},
		%x axis line style = {opacity=0},
		%ymajorgrids,
		%xticklabel style = {align=center, font=\small, rotate=60},
		%xticklabels = {Apples, Oranges, Bananas, Melons},
		%xtick style = {draw=none}, % Hide tick line
		ylabel = {RTD},
        xlabel style={align=center},
        xlabel = {Document Frequency (log scale) \\ $\xleftarrow{\textrm{More Common Words}}$\hspace{1cm}$\xrightarrow{\textrm{Less Common Words}}$},
        xmode=log,
        ymin=0.15,
        ymax=0.78,
        legend cell align=left,
        legend image post style={scale=3},
        legend pos=north east,
        legend style={draw=none},
        x dir=reverse,
		%ytick = {20, 40}
	]
		
	\addplot+[mark=*, mark options={solid}, only marks, mark size=0.5pt, blue, draw=none, opacity=0.4,
    ] table [x=Freq, y=RTD, meta=Words, col sep=comma, header=true] {redditdata.csv};

    \addlegendentry{Reddit vs SERP}

    \addplot+[mark=x, mark options={solid}, only marks, mark size=0.5pt, red, draw=none, opacity=0.5] table [x=Freq, y=Control_RTD, col sep=comma, header=true] {redditdata.csv};

    \addlegendentry{Control}

    \addplot[draw=none, fill=none, blue!20!black,
    nodes near coords*={\annotvalue},
    node near coord style={font=\footnotesize},
    visualization depends on={value \thisrow{Words} \as \annotvalue},
    each nth point={50},
    ] table [x=Freq, y=RTD, meta=Words, col sep=comma, header=true] {redditdata.csv};

		
	\end{axis}
\end{tikzpicture}

==> images/reddit_testbox.tex <==




\pgfplotstableread[col sep=space]{reddit_topbot.csv}\datatable
\pgfplotstableread[col sep=space]{reddit_bottombot.csv}\databottable


\begin{tikzpicture}
    \begin{axis}[
        width=.95\linewidth,
        height=7cm, 
        xlabel={},
        title={\textcolor{black}{Reddit}},
        xtick=\empty,
        yticklabels from table={\databottable}{x},
        ytick = {1,...,26},
        ylabel={},
        enlarge y limits={abs=2pt},
        xmin=-0.5,xmax=0.5,
        ymajorgrids,
        red,
        yticklabel style={font=\tiny, black},
        axis line style={black},
        %title={Horizontal Whisker Plot Example},
        boxplot/draw direction=x,
        boxplot/average={auto},
        boxplot/every average/.style={/tikz/mark=*,mark size=1},
    ]
\boxplotprepared{\databottable}{great}
\boxplotprepared{\databottable}{devs}
\boxplotprepared{\databottable}{items}
\boxplotprepared{\databottable}{usually}
\boxplotprepared{\databottable}{setup}
\boxplotprepared{\databottable}{recommend}
\boxplotprepared{\databottable}{cards}
\boxplotprepared{\databottable}{screen}
\boxplotprepared{\databottable}{much}
\boxplotprepared{\databottable}{issue}
\boxplotprepared{\databottable}{since}
\boxplotprepared{\databottable}{different}
\boxplotprepared{\databottable}{version}
\boxplotprepared{\databottable}{mode}
\boxplotprepared{\databottable}{works}
\boxplotprepared{\databottable}{card}
\boxplotprepared{\databottable}{settings}
\boxplotprepared{\databottable}{used}
\boxplotprepared{\databottable}{update}
\boxplotprepared{\databottable}{really}
%\boxplotprepared{\databottable}{like}
\boxplotprepared{\databottable}{game}
\boxplotprepared{\databottable}{using}
\boxplotprepared{\databottable}{would}
\boxplotprepared{\databottable}{also}
    \end{axis}
\end{tikzpicture}
\begin{tikzpicture}
    \begin{axis}[
        width=.95\linewidth,
        height=7cm, 
        xlabel style = {align=center},
        xlabel={Signed RTD \\ \textcolor{red}{$\xleftarrow{\textrm{More Likely Google}}$}\hspace{1cm}\textcolor{blue}{$\xrightarrow{\textrm{More Likely Reddit}}$}},        
        yticklabel style={font=\tiny},
        yticklabels from table={\datatable}{x},
        ytick = {1,...,26},
        ylabel={},
        xmin=-0.5,xmax=0.5,
        enlarge y limits={abs=2pt},
        ymajorgrids,
        blue,
        yticklabel style={font=\tiny, black},
        every axis label/.append style ={black},
        every tick label/.append style={black},       
        axis line style={black},        
        %title={Horizontal Whisker Plot Example},
        boxplot/draw direction=x,
        boxplot/average={auto},
        boxplot/every average/.style={/tikz/mark=*,mark size=1},
    ]
\boxplotprepared{\datatable}{removed}
\boxplotprepared{\datatable}{comments}
\boxplotprepared{\datatable}{groupbot}
\boxplotprepared{\datatable}{message}
\boxplotprepared{\datatable}{deleted}
\boxplotprepared{\datatable}{mccarthy}
\boxplotprepared{\datatable}{please}
\boxplotprepared{\datatable}{emote}
\boxplotprepared{\datatable}{refs}
\boxplotprepared{\datatable}{bengals}
\boxplotprepared{\datatable}{fuck}
\boxplotprepared{\datatable}{ukraine}
\boxplotprepared{\datatable}{mahomes}
\boxplotprepared{\datatable}{unsubscribe}
\boxplotprepared{\datatable}{hiphopheads}
\boxplotprepared{\datatable}{https}
\boxplotprepared{\datatable}{neoliberal}
\boxplotprepared{\datatable}{compose}
\boxplotprepared{\datatable}{jeffries}
\boxplotprepared{\datatable}{purdy}
\boxplotprepared{\datatable}{republican}
\boxplotprepared{\datatable}{romo}
\boxplotprepared{\datatable}{vote}
\boxplotprepared{\datatable}{jags}
\boxplotprepared{\datatable}{trump}
    \end{axis}    
\end{tikzpicture}


==> images/sent.tex <==





\begin{tikzpicture}
\begin{groupplot}[
    group style={
        group name=myplot,
        vertical sep=.2cm,
        horizontal sep=0cm,
        group size= 2 by 1
    },
    width=.6\linewidth,
    ybar,
    ymin=0.25, ymax=0.452,
    ylabel={Probability},
    xlabel={Sentiment},
    symbolic x coords={neutral,positive,negative},
    x tick label style={rotate=45, anchor=east, font=\scriptsize},
    xtick=data,
    enlarge x limits=0.5,
    legend cell align=left,
    legend image post style={scale=0.5},
    legend pos=north east,
    legend style={draw=none},
]
\nextgroupplot[title=Reddit]
\addplot+[bar width=2pt, draw=none, fill=none] 
  plot[error bars/.cd, y dir=both, y explicit]
  table[x=x,y=redditavg,y error plus expr=\thisrow{redditerr},y error minus expr=\thisrow{redditerr}] {redditsent.csv};
\addlegendentry{Reddit}
\addplot+[bar width=2pt, draw=none, fill=none] 
  plot[error bars/.cd, y dir=both, y explicit]
  table[x=x,y=serpavg,y error plus expr=\thisrow{serperr},y error minus expr=\thisrow{serperr}] {redditsent.csv};  
\addlegendentry{SERP}
\nextgroupplot[title=Twitter/X, ylabel={}, yticklabels={}]
\addplot+[bar width=2pt, draw=none, fill=none] 
  plot[error bars/.cd, y dir=both, y explicit]
  table[x=x,y=twitavg,y error plus expr=\thisrow{twiterr},y error minus expr=\thisrow{twiterr}] {twitsent.csv};
\addlegendentry{Twitter}
\addplot+[bar width=2pt, draw=none, fill=none] 
  plot[error bars/.cd, y dir=both, y explicit]
  table[x=x,y=serpavg,y error plus expr=\thisrow{serperr},y error minus expr=\thisrow{serperr}] {twitsent.csv};           
\addlegendentry{SERP}
\end{groupplot} 
\end{tikzpicture}


==> images/testbox.tex <==





\pgfplotstableread[col sep=space]{newtopavg.csv}\databottable
\pgfplotstableread[col sep=space]{newbotavg.csv}\datatable

\begin{tikzpicture}
    \begin{axis}[
        width=.84\linewidth,
        right,
        height=7cm, 
        title={\textcolor{black}{Twitter/X}},
        xlabel={},
        xtick=\empty,
        yticklabels from table={\datatable}{x},
        ytick = {1,...,26},
        ylabel={},
        enlarge y limits={abs=2pt},
        xmin=-0.5,xmax=0.5,
        ymajorgrids,
        red,
        yticklabel style={font=\tiny, black},
        axis line style={black},
        %title={Horizontal Whisker Plot Example},
        boxplot/draw direction=x,
        boxplot/average={auto},
        boxplot/every average/.style={/tikz/mark=*,mark size=1},
    ]
    
\boxplotprepared{\datatable}{mobile}
\boxplotprepared{\datatable}{ministre}
\boxplotprepared{\datatable}{cautionyespanicno}
\boxplotprepared{\datatable}{lakhs}
\boxplotprepared{\datatable}{city}
\boxplotprepared{\datatable}{minister}
\boxplotprepared{\datatable}{centre}
\boxplotprepared{\datatable}{socialsecurity}
\boxplotprepared{\datatable}{https}
\boxplotprepared{\datatable}{today}
\boxplotprepared{\datatable}{medical}
\boxplotprepared{\datatable}{communiqué}
\boxplotprepared{\datatable}{santé}
\boxplotprepared{\datatable}{dans}
\boxplotprepared{\datatable}{pour}
\boxplotprepared{\datatable}{facility}
\boxplotprepared{\datatable}{burundi}
\boxplotprepared{\datatable}{ensure}
\boxplotprepared{\datatable}{health}
\boxplotprepared{\datatable}{donated}
\boxplotprepared{\datatable}{spread}
\boxplotprepared{\datatable}{hospital}
\boxplotprepared{\datatable}{services}
\boxplotprepared{\datatable}{district}
\boxplotprepared{\datatable}{support} 
    \end{axis}
\end{tikzpicture}

\begin{tikzpicture}
    \begin{axis}[
        width=.84\linewidth,
        right,
        height=7cm, 
        xlabel style = {align=center},
        xlabel={Signed RTD \\ \textcolor{red}{$\xleftarrow{\textrm{More Likely Google}}$}\hspace{1cm}\textcolor{blue}{$\xrightarrow{\textrm{More Likely Twitter/X}}$}},
        yticklabel style={font=\tiny},
        yticklabels from table={\databottable}{x},
        ytick = {1,...,26},
        ylabel={},
        xmin=-0.5,xmax=0.5,
        enlarge y limits={abs=2pt},
        ymajorgrids,
        blue,
        yticklabel style={font=\tiny, black},
        every axis label/.append style ={black},
        every tick label/.append style={black},       
        axis line style={black},        
        %title={Horizontal Whisker Plot Example},
        boxplot/draw direction=x,
        boxplot/average={auto},
        boxplot/every average/.style={/tikz/mark=*,mark size=1, red},
    ]
\boxplotprepared{\databottable}{coronavirusupdate}
\boxplotprepared{\databottable}{trump}
\boxplotprepared{\databottable}{deaths}
\boxplotprepared{\databottable}{coronaviruspandemic}
\boxplotprepared{\databottable}{death}
\boxplotprepared{\databottable}{china}
\boxplotprepared{\databottable}{corona}
\boxplotprepared{\databottable}{quarantinelife}
\boxplotprepared{\databottable}{coronavirustruth}
\boxplotprepared{\databottable}{realdonaldtrump}
\boxplotprepared{\databottable}{coronavirususa}
\boxplotprepared{\databottable}{stayhome}
\boxplotprepared{\databottable}{coronaupdate}
\boxplotprepared{\databottable}{stayathome}
\boxplotprepared{\databottable}{stayathomeandstaysafe}
\boxplotprepared{\databottable}{coronavirusuk}
\boxplotprepared{\databottable}{evdekal}
\boxplotprepared{\databottable}{youtube}
\boxplotprepared{\databottable}{coronavirusupdates}
\boxplotprepared{\databottable}{chinesevirus}
\boxplotprepared{\databottable}{coronavirusinpakistan}
\boxplotprepared{\databottable}{trumpvirus}
\boxplotprepared{\databottable}{lockdowneffect}
\boxplotprepared{\databottable}{stayathomesavelives}
\boxplotprepared{\databottable}{coronaupdatesinindia}
    \end{axis}
\end{tikzpicture}



==> images/twitter_rtd.tex <==


\begin{tikzpicture}
	\begin{axis}[
        width=\linewidth,
        height=2.5in,
        title={Twitter/X},
		%x axis line style = {opacity=0},
		%ymajorgrids,
		%xticklabel style = {align=center, font=\small, rotate=60},
		%xticklabels = {Apples, Oranges, Bananas, Melons},
		%xtick style = {draw=none}, % Hide tick line
		ylabel = {RTD},
        xlabel style={align=center},
        xlabel = {Document Frequency (log scale) \\ $\xleftarrow{\textrm{More Common Words}}$\hspace{1cm}$\xrightarrow{\textrm{Less Common Words}}$},
        xmode=log,
        ymin=0.3,
        ymax=1.00,
        legend cell align=left,
        legend image post style={scale=3},
        legend pos=north east,
        legend style={draw=none},
        x dir=reverse,
		%ytick = {20, 40}
	]
		
	\addplot+[mark=*, mark options={solid}, only marks, mark size=0.5pt, blue, draw=none, opacity=0.4,
    ] table [x=Freq, y=RTD, meta=Words, col sep=comma, header=true] {twitterdata.csv};

    \addlegendentry{Twiter/X vs SERP}

    \addplot+[mark=x, mark options={solid}, only marks, mark size=0.5pt, red, draw=none, opacity=0.5] table [x=Freq, y=Control_RTD, col sep=comma, header=true] {twitterdata.csv};

    \addlegendentry{Control}

    \addplot[draw=none, fill=none, blue!20!black,
    nodes near coords*={\annotvalue},
    node near coord style={font=\footnotesize},
    visualization depends on={value \thisrow{Words} \as \annotvalue},
    each nth point={52},
    ] table [x=Freq, y=RTD, meta=Words, col sep=comma, header=true] {twitterdata.csv};

		
	\end{axis}
\end{tikzpicture}
